Some prospects for semiproducts and products of modal logics

We consider products and semiproducts of propositional modal logics L with S5 and present new examples of product and semiproduct logics axiomatized in the minimal way and enjoying the product (or semiproduct) FMP. An essential part of the proof is local tabularity of these (semi)products for L of finite depth; it is obtained by using bisimulation games. These results readily imply decidability for 1-variable fragments of predicate modal logics QL and QL+Barcan formula. We also present new counterexamples, i.e. (semi)products not axiomatizable in the simplest way.

==> jsinputs.tex <==

\newcommand{\loopr}{\looparrowright}

\newcommand{\quotes}[1]{\mbox{``}#1\mbox{''}}
%\newcommand{\LNCS}{\mbox{\em Lecture Notes in Computer Science}}
\newcommand{\success}{\mbox{\em Success}}

% to automatically change less than and greater than to math angle brackets:
%\mathcode`\<=''4268 % < = \langle
%\mathcode`\>=''5269 % > = \rangle

%% double bigwedge and double bigvee,
%% both having the option of centered, displayed subscripts and superscripts 
\newcommand{\dwedge}[2]%
{\overset{#1}{\underset{#2}{\mbox{$\bigwedge\hspace{-2ex}\bigwedge$}}}}
\newcommand{\dvee}[2]%
{\overset{#1}{\underset{#2}{\mbox{$\bigvee\hspace{-2ex}\bigvee$}}}}


%% double times and double plus (like a hash, but square)
%% Visser's chapter in the Handbook of Phil Log
%% use pstricks
\newcommand{\dplus}
{\mbox{{\unitlength0.08mm
\begin{picture}(30,35)
\put(0,10){\line(1,0){30}}
\put(0,20){\line(1,0){30}}
\put(10,0){\line(0,1){30}}
\put(20,0){\line(0,1){30}}
\end{picture}}}}



\newcommand{\dcross}
{{\psset{unit=1mm}\mbox{\rput{45}(1,1.2){\dplus}\hspace{2.4mm}}}}


\newcommand{\corners}[1]{\ulcorner {#1}\urcorner}
\newcommand{\jset}[1]{\langle {#1}\rangle}
\newcommand{\jsem}[1]{\lsem {#1}\rsem}
%% js \newcommand{\citedef}[1]{\ \hspace{-1pt}{\rm \cite{#1}}}

% use this to define new macros, eg:
% \newcommand{\Hi}{\inMath{\cal A}}
% it will check whether you are in math mode or not, and 
% deal with the macro accordingly.
% * in plain text, must be followed by punctuation, or \ blank. **
\newcommand{\inMath}[1]{\relax\ifmmode{#1}%
\else{\mbox{$#1$}}\fi}


%\cross produces a stretchable diagonal line for the text within {}
%% eg:  \cross{Alpha} produces a crossed-out "Alpha"
%% needs pstricks and pst-node in the documentstyle argument to work.
%% specially produced by H-J Ohlbach for Sundholm's formulae in HBPL

%% zigzag, and botdot and boxarrow all need pstricks in documentstyle

\newcommand{\vdot}%
{\unitlength0.4mm
\begin{picture}(8,10)
\put(4,0){.}
\put(0,10){.}
\put(8,10){.}
\put(2,5){.}
\put(6,5){.}
\end{picture}
}

\newcommand{\ignore}[1]{}
%% ignores all text inside curly brackets when 
%% LaTeX is run:  \ignore{this text}.

\def\fishook{\,{\vrule width2ex height0.85ex depth-0.75ex}\!\!{\sf 3}\,}
%%which I got from Herb Enderton    (hbe@math.ucla.edu)
%%Antoni Diller

%% produces a curled right arrow for various chapters in HPL
%% js \newcommand{\fishook}{\mathbin{
%% js \unitlength1ex
%% js \psset{unit=\unitlength,linewidth=0.4pt}
%% js \raisebox{0.5ex}{\begin{picture}(2,1)
%% js \psbezier(0.7,0)(3.2,0)(1.5,1.6)(1.3,0.6)
%% js \psbezier(0.7,0)(3.2,0)(1.5,-1.6)(1.3,-0.6)
%% js \psline(0,0)(1,0)
%% js \end{picture}
%% js }}}

\newcommand{\sfishook}{\scalebox{0.7}{\fishook}}

\newcommand{\botdot}{\mbox{
%%%\bbot from HJO Sept 96
\raisebox{0.1mm}{\mbox{\unitlength1mm
\begin{picture}(2.5,2)
\put(0,0){\line(1,0){2.4}}
\put(0.8,0){\line(0,1){2.2}}
\put(1.6,0){\line(0,1){2.2}}
\put(0.75,1){.}
\end{picture}}}}}

\newcommand{\boxto}{% \barrow from HJO Sept 96
\mathbin{\mbox{\psset{unit=0.1mm}
\psframe[linewidth=0.4pt](0,1)(15,16)~$\rightarrow$}}}

%%Hans Juergen's special itemized environment for 
%lists with roman counters.  USE "mylist", not enumerate!!
%% see page 75 of LaTeX2e manual for variations
%%\newcounter{mylistcounter}
%%\newenvironment{mylist}%
%%{\setcounter{mylistcounter}0
%%\begin{list}{\roman{mylistcounter})}{\usecounter{mylistcounter}
%%\itemsep0mm \parsep0mm \topsep0pt \listparindent0pt 
%%\labelwidth7mm 
%%\labelsep2mm}}%
%%{\end{list}}

%%HJ's \ref command to complement roman lists.
\newcommand{\romanref}[1]{%
\if \ref{#1}\empty {\setcounter{romanrefcounter}0} \else 
{\setcounter{romanrefcounter}{\ref{#1}}}\fi%
{\it \roman{romanrefcounter}}}


%%\newcommand{\dashV}{-\!\!\!\|\, }%% gets \dashV
%%\newcommand{\Dashv}{=\joinrel\mathrel|}%% gets \Dashv
%% from Maarten de Rijke 5.9.96

\newcommand{\TO}{\twoheadrightarrow}
\newcommand{\ninth}{\mbox{$\frac{1}{9}$}}
\newcommand{\sixth}{\mbox{$\frac{1}{6}$}}
\newcommand{\quarter}{\mbox{$\frac{1}{4}$}}
\newcommand{\twoninths}{\mbox{$\frac{2}{9}$}}
\newcommand{\twofifths}{\mbox{$\frac{2}{5}$}}
\newcommand{\threefifths}{\mbox{$\frac{3}{5}$}}
%\newcommand{\half}{\mbox{$\frac{1}{2}$}}
%%\newcommand{\third}{\mbox{$\frac{1}{3}$}}
%%\newcommand{\ddiv}{\mbox{$\dot{-}$}} 
\newcommand{\ddiv}{\mbox{$-{\hspace{-.55em}\raisebox{1ex}{.}}$}}

%%\newcommand{\eqref}[1]{(\ref{#1})}

%%\newcommand{\set}[1]{\langle #1 \rangle}

%%\newcommand{\cross}[1]{
        %%\pnode{crossa}
        %%#1$\!\!$
        %%\raisebox{1.5ex}{\pnode{crossb}}$\;\;$
        %%\ncline{-}{crossa}{crossb}
        %%}
\newcommand{\cross}[1]{{\psset{linewidth=.15pt}%
        \pnode{crossa}%
        #1$\!$%
        \raisebox{1.5ex}{\pnode{crossb}}$\;\;$%
        \ncline{-}{crossa}{crossb}$\!\!$%
        }}

\newcommand{\BA}{{\bf A}}
\newcommand{\BBA}{\mbox{\(\mathbb{ A}\)}}
\newcommand{\Ba}{{\bf a}}
\newcommand{\uA}{{\underline A}}
\newcommand{\Ua}{{\underline a}}
\newcommand{\Ub}{{\underline b}}
\newcommand{\UB}{{\underline{B}}}
\newcommand{\Uc}{{\underline c}}
\newcommand{\Ud}{{\underline d}}
\newcommand{\Ux}{{\underline x}}
\newcommand{\Uy}{{\underline y}}
\newcommand{\Uz}{{\underline z}}

\newcommand{\CA}{{\cal A}}
\newcommand{\BB}{{\bf B}}
\newcommand{\BBB}{\mbox{\(\Bbb B\)}}
\newcommand{\Bb}{{\bf b}}
\newcommand{\Bc}{{\bf c}}
\newcommand{\CB}{\mathcal{B}}
\newcommand{\BC}{{\bf C}}
\newcommand{\CC}{\mbox{$\mathcal{C}$}}
\newcommand{\BBC}{\mbox{\(\Bbb C\)}}
\newcommand{\BD}{{\bf D}}
\newcommand{\CD}{\mbox{$\mathcal{D}$}}
\newcommand{\Bd}{{\bf d}}
\newcommand{\BBD}{\mbox{\(\Bbb D\)}}
\newcommand{\BBE}{\mbox{\(\Bbb E\)}}
\newcommand{\CE}{\mbox{$\mathcal{E}$}}
\newcommand{\BE}{{\bf E}}
\newcommand{\Be}{{\bf e}}
%%\newcommand{\BF}{\mbox{{\bf F}}}
\newcommand{\BF}{{\bf F}} 
\newcommand{\CF}{\mathcal{F}}
\newcommand{\BBF}{\mbox{\(\mathbb{F}\)}}
\newcommand{\Bf}{{\bf f}}
\newcommand{\Sf}{{\sf f}}
\newcommand{\BG}{{\bf G}}
\newcommand{\BBG}{\mbox{\(\Bbb G\)}}
\newcommand{\Bg}{{\bf g}}
\newcommand{\BH}{{\bf H}}
\newcommand{\Bh}{{\bf h}}
\newcommand{\uh}{\underline{h}}
\newcommand{\CH}{{\cal H}}
\newcommand{\BBH}{\mbox{\(\Bbb H\)}}
\newcommand{\BBI}{\mbox{\(\Bbb I\)}}
\newcommand{\CI}{{\mathcal I}}
\newcommand{\BI}{{\bf I}}
\newcommand{\Bi}{{\bf I}}
\newcommand{\Bj}{{\bf j}}
\newcommand{\BJ}{{\bf J}}
\newcommand{\CJ}{\mathcal{J}}
\newcommand{\BBJ}{\mbox{\(\Bbb J\)}}
\newcommand{\BK}{{\bf K}}
\newcommand{\CK}{{\cal K}}
\newcommand{\Bk}{{\bf k}}
\newcommand{\BBK}{\mbox {\(\Bbb K\)}}
\newcommand{\BL}{{{\bf L}}}
\newcommand{\CL}{{\mathcal{L}}}
\newcommand{\BBL}{\mbox{\(\Bbb L\)}}
\newcommand{\Bl}{{\bf l}}
\newcommand{\UL}{\underline {\Lambda}}
\newcommand{\BLL}{{\bf LL}}
\newcommand{\BM}{{\bf M}}
\newcommand{\UM}{\underline{M}}
\newcommand{\CM}{{\mathcal{M}}}
\newcommand{\BBM}{\mbox{\(\Bbb M\)}}
\newcommand{\Bm}{{\bf m}}
\newcommand{\BN}{{\bf N}}
\newcommand{\Bn}{{\bf n}}
\newcommand{\BBN}{\mbox{\(\Bbb N\)}}
\newcommand{\un}{\underline n}
\newcommand{\CN}{{\mathcal N}}
\newcommand{\BO}{{\bf O}}
\newcommand{\Bo}{{\bf o}}
\newcommand{\CO}{{\mathcal O}}
\newcommand{\BBP}{\mbox{\(\Bbb P\)}}
%\newcommand{\UP}{\underline{P}}

\newcommand{\CP}{\mbox{$\mathcal{P}$}}
\newcommand{\BP}{{\bf P}}
\newcommand{\Bp}{{\bf p}}
\newcommand{\TP}{\tilde{P}}
%\newcommand{\Tp}{\tilde{p}}
\newcommand{\UP}{{\underline{P}}}
\newcommand{\upi}{\underline{\pi}}
\newcommand{\BPi}{{\bf \Pi}}
\newcommand{\Bq}{{\bf q}}
\newcommand{\BQ}{{\bf Q}}
\newcommand{\UQ}{\underline{Q}}
\newcommand{\BBQ}{\mbox{\(\Bbb Q\)}}
\newcommand{\RR}{{\rm R}}
\newcommand{\BR}{{\bf R}}
\newcommand{\Br}{{\bf r}}
\newcommand{\CR}{{\cal R}}
\newcommand{\BBR}{\mbox{\(\Bbb R\)}}
\newcommand{\CS}{{\mathcal{S}}}
\newcommand{\BS}{{\bf S}}
\newcommand{\Bs}{{\bf s}}
\newcommand{\BBS}{\mbox{\(\Bbb S\)}}
\newcommand{\BT}{{\bf T}}
\newcommand{\CT}{\mathcal{T}}
\newcommand{\BBT}{\mbox{\(\Bbb T\)}}
\newcommand{\Ut}{\underline{t}}
\newcommand{\Bt}{{\bf t}}
\newcommand{\BV}{{\bf V}}
\newcommand{\BU}{{\bf U}}

\newcommand{\CU}{{\mathcal{U}}}
\newcommand{\BBU}{\mbox{\(\Bbb U\)}}
\newcommand{\Uu}{\underline{u}}
\newcommand{\Bu}{{\bf u}}
\newcommand{\BBV}{\mbox{\(\Bbb V\)}}
\newcommand{\Uv}{\underline{v}}
\newcommand{\Bv}{{\bf v}}
\newcommand{\BW}{{\bf W}}
\newcommand{\Uw}{\underline{w}}
\newcommand{\Bw}{{\bf w}}
\newcommand{\BBW}{\mbox{\(\Bbb W\)}}
\newcommand{\Bx}{{\bf x}}
\newcommand{\BBX}{\mbox{\(\Bbb X\)}}
\newcommand{\BX}{{\bf X}}
\newcommand{\By}{{\bf y}}
\newcommand{\BY}{{\bf Y}}
\newcommand{\BBY}{\mbox{\(\Bbb Y\)}}
\newcommand{\Bz}{{\bf z}}
\newcommand{\BZ}{{\bf Z}}
\newcommand{\BBZ}{\mbox{\(\Bbb Z\)}}

\newcommand{\doublewedge}{\mathbin{\bigwedge \hspace{-.85em}\bigwedge}}
\newcommand{\doublevee}{\mathbin{\bigvee \hspace{-.85em}\bigvee}}

%% see DRUMS 4 Abduction chapter
%% Black hole symbol
%%\[\begin{array}{l}
%%\Delta, X, \bigoall{X} = \Delta.\\
%%\doublecirc \hspace*{-.41cm}\raisebox{.02ex} X = X 
%%\end{array}
%%\]
\newlength{\circlen}
\newlength{\symblen}
\newcommand{\bigoall}[1]{\settowidth{\circlen}{$\bigcirc$}%
\settowidth{\symblen}{$#1$}%
\setlength{\circlen}{-0.6\circlen}%
\addtolength{\circlen}{-0.6\symblen}%
\mbox{\Large$\bigcirc$\normalsize\hspace*{\circlen}{$#1$}}\ %
}

\newcommand{\doublecirc}{\text{\raisebox{-2.5pt}{\SmallCircle\llap{\BigCircle}$\,$}}}


%\newcommand{\doublecirc}{
%\mbox{\Large$\bigcirc$\normalsize\hspace*{-2.8ex}{\raisebox{0.35mm}{$\bigcirc$}}}\ %
%}

%\newcommand{\oall}[1]{\settowidth{\circlen}{$\bigcirc$}%
%\settowidth{\symblen}{$#1$}}
\newcommand{\oallsymb}{\w{$\bigcirc$}} 
\newcommand{\oall}[1]{\mbox{$\bigcirc (#1)$}}
\renewcommand{\bigoall}{\oall}
\newcommand{\dbh}[1]{\doublecirc (#1)}
\newcommand{\insquare}[1]{\mbox{$\square \hspace*{-1.5ex}\raisebox{.4ex}{\mbox{{\tiny#1}}}$}}
\newcommand{\incircle}[1]{\mbox{$\bigcirc \hspace*{-2.2ex}\raisebox{.4ex}{\mbox{{\tiny#1}}}$}}


%% some things from Odinaldo used for Belief Contraction paper
\newcommand{\antiwff}{\w{\bigoall{~}}}
\newcommand{\circled}[1]{\w{\bigoall{#1}}}
\newcommand{\ncircled}[2]{\w{$\bigoall{#2}^{#1}$}}
\newcommand{\prog}[1]{\texttt{\small #1}}
%\newcommand{\contsymb}{\w{$-$}}
\newcommand{\contract}[2]{\w{$#1 \contsymb #2$}}
%\newcommand{\postulate}[1]{\noindent{\bf #1:}\\}
\newcommand{\w}[1]{\text{#1}}
\newcommand{\ws}[1]{~\text{#1}~}
\ifx\text\undefined
  \newcommand{\text}[1]{\relax
    \ifmmode\mathchoice
      {\hbox{\the\textfont0\relax#1}}%
      {\hbox{\the\textfont0\relax#1}}%
      {\hbox{\the\scriptfont0\relax#1}}%
      {\hbox{\the\scriptscriptfont0\relax#1}}%
    \else{\relax#1}\fi}
  \fi

\newcommand{\pr}{\w{$^{\prime}$}}
\newcommand{\statement}[2]{\noindent\parbox{1.2cm}{#1}#2}
\newcommand{\agmconsymb}{\w{$-$}}
\newcommand{\agmexpsymb}{\w{$+$}}
\newcommand{\agmrevsymb}{\w{$*$}}
\newcommand{\n}[2]{\w{${#2}^{#1}$}}
\newcommand{\agmcon}[2]{\w{${#1}^{\agmconsymb}_{#2}$}}
\newcommand{\contraction}[2]{\w{${#1}^{\consymb}_{#2}$}}
\newcommand{\revision}[2]{\w{${#1}^{\revsymb}_{#2}$}}
\newcommand{\agmexp}[2]{\w{${#1}^{\agmexpsymb}_{#2}$}}
\newcommand{\agmrev}[2]{\w{${#1}^{\agmrevsymb}_{#2}$}}
\newcommand{\consymb}{\agmconsymb}
\newcommand{\revsymb}{\agmrevsymb}
\newcommand{\defitem}[1]{#1}
\newcommand{\defitemkey}[2]{#1}
\newcommand{\defsub}[1]{}
\newcommand{\defsym}[1]{#1}
\newcommand{\defent}[1]{#1}
\newcommand{\defentkey}[2]{#2}


%%from HJO 12.8.97 for look.tex
\newcommand{\lozengeminus}{%
\mbox{\unitlength1mm
\begin{picture}(0,0)
\put(0.2,1){\line(1,0){1.8}}
\end{picture}$\lozenge$}}


%%\newlength{\squaren}
%%%%\newlength{\symblen}
%%\newcommand{\boxall}[1]{\settowidth{\squaren}{$\square$}%
%%\settowidth{\symblen}{$#1$}%
%%\setlength{\squaren}{-0.5\squaren}%
%%\addtolength{\squaren}{-0.5\symblen}%
%%\mbox{$\square$\hspace*{\squaren}{$#1$}}%
%%}

% HJO's command for putting variables inside a box.
% needs pstricks to work.
\newcommand{\boxall}[2]{%
\psframebox[framesep=1pt]{\parbox{#2}{\centering#1}}}


\newcommand{\obang}{\mbox{$\bigcirc \hspace{-0.75em} !$}}
%%\newcommand{\owedge}{\mbox{$\bigcirc \hspace{-0.85em} \wedge$}}
%%\newcommand{\ovee}{\mbox{$\bigcirc \hspace{-0.85em} \vee$}}
%\newcommand{\Ct}{\mbox{$\bigcirc \hspace{-0.75em} {\footnotesize{M}}$}}
%%\newcommand{\Ct}{\mbox{ $\bigcirc$ \hspace*{-1.15em}{\tiny{M}} }}
\newcommand{\Ct}{\mbox{$\oall{{\footnotesize M}}$}}
\newcommand{\double}{\mbox{{\raisebox{.2ex}{\small $\,=\!\!\!| |\!\!\!=\,$}}}}

\newcommand{\proves}{\mbox{${\mid\!\sim}$}}
\newcommand{\nproves}{\mid\!\not\sim}
%%\newcommand{\proves}{\mathbin{\mbox{\raisebox{0.5mm}{\scalebox{0.75}{$\mid\!\sim$ }}}}}

\newcommand{\thr}{\twoheadrightarrow}
\newcommand{\To}{\Rightarrow}

\newcommand{\zigzag}{%
\mathbin{\raisebox{-0.5mm}%
{\mbox{\unitlength1mm\psset{unit=\unitlength}%
\begin{picture}(3.5,2)%
\put(0,0){$\leftarrow$}%
\put(0,2){$\rightarrow$}%
\psline[linewidth=0.4pt](3.2,0.9)(0.2,2.9)%
\end{picture}}}}}

\newcommand{\IO}{{\sl On}}
\newcommand{\IM}{{\sl Move}}
\newcommand{\IF}{{\sl Free}}
\newcommand{\QA}{{\cal Q}_{\mbox{\scriptsize{\em Abduce}}}} 
\newcommand{\boxa}{{\fbox{a}}} \newcommand{\vdashtilde}{\mid \!\sim}
\newcommand {\Proves}   {\mathrel{\mbox{$|\mkern-8.4mu\sim$}}}

\newcommand{\lsem}{[\![}
\newcommand{\rsem}{]\!]}
\newcommand{\eside}{\mbox{${\cup \hspace {-1.8ex} \shortmid}$~}}
\newcommand{\upar}{{\|\hspace{-.41em}{\rule[-0.6ex]{1.3ex}{0.4pt}}}}

\newcommand{\myfrac}[2]{\displaystyle\frac{#1}{#2}}
\newcommand{\jqed}{\hfill \rule{1.3217ex}{2ex}} %%$\blacksquare$} %\rule{2mm}{3mm}}
\newcommand{\Star}{{*}}
\newcommand{\BPS}{{\bf P}{\rm\/S}}
\newcommand{\nin}{{\not\in}}
\newcommand{\vertnto}{{\to \hspace{-1.5ex} \shortmid}}

% command to force early end of proof marker. This is used if the end
% of proof marker would otherwise come out in the wrong place.
%%\def\qed{\xqed\global\SuppressEndOfProoftrue}
%%\newif\ifSuppressEndOfProof\SuppressEndOfProoffalse
%%\def\xqed{\pushright\markendofproof}
%%\def\markendofproof{\rule{1.3217ex}{2ex}}
%

\newcommand{\lambdachurch}{$\lambda{\rightarrow}$-Church}
\newcommand{\lambdacurry}{$\lambda{\rightarrow}$-Curry}
\newcommand{\Ubeta}{\underline{\beta}}


\def\maxk{\mathop{k{\rm Max}}\displaylimits}

\def\twoheaddownarrow{\rlap{$\downarrow$}\raise-.5ex\hbox{$\downarrow$}}%%
\def\twoheaduparrow{\rlap{$\uparrow$}\raise.5ex\hbox{$\uparrow$}}%%

\def\texturespicture #1 by #2 (#3){
\vbox to #2 {\hrule width #1 height 0pt depth 0pt
}}
%\vfill \special{psfile="#3"}

\def\scaledpicture #1 by #2 (#3 scaled #4){{\dimen0=#1 \dimen1=#2
\divide\dimen0 by 1000 \multiply \dimen0 by #4
\divide\dimen1 by 1000 \multiply \dimen1 by #4
\texturespicture\dimen0 by \dimen1 (#3 scaled #4)}}


%to position picture at correct position in file
%\begin{center}
%\hspace{3.5cm}{\scaledpicture 2.54in by 0.93in (Fig1 scaled 1000)}
%where figures are the sizes of the actual figures in .picture file
% caption{Figure 1}
%\end{center}

% environment for Dov's boxes
\newenvironment{Dovbox}[1]%
 {\begin{tabular}[t]{llr} && \fbox{#1}\\}%
 {\end{tabular}}

%% js % environments for theorems, definitions, propositions, etc		       
%% \newtheorem{theorem}{Theorem}[section]					       
%% js \newtheorem{definition}[theorem]{Definition}				          \newtheorem{placeholder}[theorem]{}


%% js \newtheorem{case}[theorem]{Case}					       
%% js \newtheorem{proposition}[theorem]{Proposition}				       
%% \newtheorem{exercise}[theorem]{Exercise}				       
%% js \newtheorem{construction}[theorem]{Construction}			       
%% js \newtheorem{problem}[theorem]{Problem}					       
%% js \newtheorem{corollary}[theorem]{Corollary}				       
%% js \newtheorem{claim}[theorem]{Claim}					       
%% js \newtheorem{lemma}[theorem]{Lemma}					       
%% js \newtheorem{fact}[theorem]{Fact}					       
%% js \newtheorem{elimination}[theorem]{Elimination}				       
%% js \newtheorem{remark}[theorem]{Remark}					       
%% js \newtheorem{observation}[theorem]{Observation}				       
%% js \newtheorem{remarks}[theorem]{Remarks}					       
%% js \newtheorem{example}[theorem]{Example}					       
%% js \newtheorem{summary}[theorem]{Summary}					       
%% js \newtheorem{examples}[theorem]{Examples}				       
%% js \newtheorem{plenitude}[theorem]{Plenitude}				       
%% js \newtheorem{singletons}[theorem]{Singletons}	
			       
%% js %%%%									       
%% js %%									       
%% js 										     
% for Linz \newenvironment{proof}{\begin{trivlist}\item[]{\bf Proof.}}{\hspace*{\fill} $\blacksquare$ \end{trivlist}}
  
%%%%%%%%\newcommand{\eproof}{\hspace*{\fill} $\blacksquare$}
%%%%%%
%%% environment for the columnated examples
%\newenvironment{example}{\begin{trivlist}
%\addtolength{\leftmargin}{0.5in}
%\item[]
%\begin{tabular}{p{2in}l}}%
%{\end{tabular}
%\end{trivlist}}

\newenvironment{defnlist}{\begin{list}{}{\setlength{\parsep}{0em}%
\setlength{\parskip}{0em}\setlength{\listparindent}{0em}}}%
{\end{list}}

\newenvironment{data}{\begin{trivlist}%
\addtolength{\leftmargin}{0.5in}%
\item[]%
\begin{tabular}{p{2in}c}%
{\bf Data}&{\bf original goal}\\}%
{\end{tabular}%
\end{trivlist}}

\input prooftree
\newcommand \prt [3] {\prooftree #1 \justifies #2
\using #3 \endprooftree}

\newcommand\Prt [3] {\prooftree#1 \Justifies #2 \using #3\endprooftree}


\newcommand{\jnotind}[1]{\notind{#1}#1} %rjq 10.11.92
%\newcommand{\jnotind}[1]{#1\notind{#1}}
\newcommand{\jauind}[1]{\auind{#1}#1} %rjq 10.11.92
%\newcommand{\jauind}[1]{#1\auind{#1}}
\newcommand{\jsubind}[1]{\subind{#1}#1} %rjq 10.11.92
%\newcommand{\jsubind}[1]{#1\subind{#1}}

% print (maths) text and strike though it horizontally
\newcommand\strikethrough[1]{{\setbox0=\hbox{$#1$}
\hrule height.75ex depth-.65ex width\wd0 \kern-\wd0\box0}}

% make <> into brackets, and back into less/greater
\newcommand\makeanglebrackets{\mathcode`\<="4268 \mathcode`\>="5269 }
\newcommand\makelessgreater{\mathcode`\<="313C \mathcode`\>="313E }
\mathchardef\gt="313E \mathchardef\lt="313C

\input{rotate.tex}
\newsavebox{\iotabox}
\savebox{\iotabox}{$\iota$}
\newsavebox{\updowniota}
\savebox{\updowniota}{\rotu\iotabox}
\newcommand{\atoi}{\usebox{\updowniota}}

%% js \newsavebox{\arrowbox}
%% js \savebox{\arrowbox}{$\ding{225}$}
%% js \newsavebox{\newdownarrow}
%% js \savebox{\newdownarrow}{\rotr\arrowbox}
%% js \newcommand{\newDownarrow}{\usebox{\newdownarrow}}


\newsavebox{\ampersandbox}
\savebox{\ampersandbox}{$\&$}
\newsavebox{\updownampersand}
\savebox{\updownampersand}{\rotu\ampersandbox}
\newcommand{\Par}{\usebox{\updownampersand}}


%\newcommand{\mapsfrom}{{\leftarrow \!\!\!|~}}

%%\newsavebox{\mapstobox}
%%\savebox{\mapstobox}{$\mapsto$}
%%\newsavebox{\backwardsmapsto}
%%\savebox{\backwardsmapsto}{\rotu\mapstobox}
%%\newcommand{\mapsfrom}{\usebox{\backwardsmapsto}}



\newcommand{\jmax}{\mbox{ max}}
\newcommand{\plus}{+\cdots +}
\newcommand{\comma}{,\ldots ,}


\newcommand{\jand}{\mathop{{\&}}\limits}
\newcommand{\jX}{\mathop{X}\limits}

% for Agenda Relevance, chapter 15
\newcommand{\bigsquare}{{\Large\square}}
\newcommand{\barsquare}{\mbox{$\bigsquare\!\!\! |$}}
\newcommand{\barlozenge}{\mbox{$\large\lozenge \!\!\! |$}}
\newcommand{\now}{{\mbox{\em now}}}


%For Agenda Relevance, chapter 15
\def\barsquare{{\hbox{\begin{turn}{90}$\boxminus$\end{turn}}}}
\def\barlozenge{{\hbox{$\lozenge$\hspace{-4.7pt}\vspace{-2pt}\raisebox{1.1pt}{\scriptsize{$|$}}%
\hspace{4.7pt}\vspace{2pt}}}}

%% paper 256
\def\undern#1{\vtop{\ialign{##\crcr
 $\hfil\displaystyle{#1}\hfil$\crcr
 \noalign{\kern-.1pt\nointerlineskip}%
 ~\,\raisebox{-.5ex}{$n \to \infty$} \crcr}}}
\def\Limn{\mathop{\undern{\sf Lim}}\displaylimits}


%% paper260
\newcommand{\attack}{\mbox{ Attack}}

\newcommand{\infx}{\displaystyle\inf_{x}}
\newcommand{\infi}{\displaystyle\inf_{i}}
\newcommand{\mini}{\displaystyle\min_{i}}
\newcommand{\supx}{\displaystyle\sup_{x}}

%% js \def\undern#1{\vtop{\ialign{##\crcr
%% js  $\hfil\displaystyle{#1}\hfil$\crcr
%% js  \noalign{\kern-.1pt\nointerlineskip}%
%% js  ~\,\raisebox{-.5ex}{$x$} \crcr}}}
%% js \def\infx{\mathop{\undern{\sf Infimum}}\displaylimits}
%% js 
%% js \def\undern#1{\vtop{\ialign{##\crcr
%% js  $\hfil\displaystyle{#1}\hfil$\crcr
%% js  \noalign{\kern-.1pt\nointerlineskip}%
%% js  ~\,\raisebox{-.5ex}{$i$} \crcr}}}
%% js \def\infi{\mathop{\undern{\sf Infimum}}\displaylimits}
%% js 
%% js \def\undern#1{\vtop{\ialign{##\crcr
%% js  $\hfil\displaystyle{#1}\hfil$\crcr
%% js  \noalign{\kern-.1pt\nointerlineskip}%
%% js  ~\,\raisebox{-.5ex}{$i$} \crcr}}}
%% js \def\mini{\mathop{\undern{\sf min}}\displaylimits}
%% js 
%% js 
%% js \def\undern#1{\vtop{\ialign{##\crcr
%% js  $\hfil\displaystyle{#1}\hfil$\crcr
%% js  \noalign{\kern-.1pt\nointerlineskip}%
%% js  ~\,\raisebox{-.5ex}{$x$} \crcr}}}
%% js \def\supx{\mathop{\undern{\sf Supremum}}\displaylimits}


%paper 257
\newcommand{\exit}{\mbox{Exit}}

\def\undern#1{\vtop{\ialign{##\crcr
 $\hfil\displaystyle{#1}\hfil$\crcr
 \noalign{\kern-.1pt\nointerlineskip}%
 ~\,\raisebox{-.5ex}{$i$} \crcr}}}
\def\supi{\mathop{\undern{\sf Sup}}\displaylimits}

\newcommand{\vare}{\varepsilon}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> vsinputs.tex <==
%\renewcommand{\baselinestretch}{1.5}
%\renewcommand{\baselinestretch}{2}
% environments for theorems, definitions, propositions, etc
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{case}[theorem]{Case}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{exercise}[theorem]{Exercise}
%\newtheorem{construction}[theorem]{Construction}
%\newtheorem{problem}[theorem]{Problem}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{fact}[theorem]{Fact}
%\newtheorem{elimination}[theorem]{Elimination}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{observation}[theorem]{Observation}
%\newtheorem{remarks}[theorem]{Remarks}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{summary}[theorem]{Summary}
%\newtheorem{examples}[theorem]{Examples}
%\newtheorem{plenitude}[theorem]{Plenitude}
%\newtheorem{singletons}[theorem]{Singletons}
%\newenvironment{proof}{\begin{trivlist}\item[]{\bf Proof\ \ }}
%{\hspace*{\fill} $\blacksquare$ \end{trivlist}}

%\renewcommand{\labelenumi}{(\roman{enumi})}
%\newcommand{\lbu}{\bullet}
%\newcommand{\mathbb}[1]{\Bbb{#1}}
%\newcommand{\two}{\mbox{\small\psframebox[framesep=0.4mm]{2}}}
%\newfont{\bi}{cmmib10}
%\newtheorem{coro}[theorem]{Corollary}
%\newtheorem{defi}[theorem]{Definition}
%\newtheorem{lem}[theorem]{Lemma}
%\newtheorem{propo}[theorem]{Proposition}
%\newtheorem{que}[theorem]{Question}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{theo}{Theorem}[section]

%\def\b{\beta}
%\newcommand\bfi[1]{\hbox{\textbf{\itshape #1}}}
\def\bmH{\boldmath\mbox{\bf H}\unboldmath}
\def\bo{{\mbox{\bf 1}}}
\def\bz{{\mbox{$\boldsymbol z$}}}
\def\<{\langle}
\def\>{\rangle}
\def\AoAk{{A_1,\dots,A_k}}
\def\Lrarr{{\Leftrightarrow}}
\def\MFa{{MF_{T'}^{(=)}}}
\def\nvd{{\not\vdash}}

\def\AoAm{{A_0,\dots,A_m}}
\def\AoAn{{A_0,\dots,A_n}}
\def\AowAm{{A_0\wedge A_m}}
\def\aoan{{a_1,\dots,a_n}}
\def\a1an{{a_1,\dots,a_n}}
\def\nVd{\,\not\Vdash\,}
\def\al{\alpha}
\def\al{\alpha}
\def\alp{\alpha}
%\def\and{~\&~}
\def\conj{~\&~}
\def\app{\approx}
\def\as{\asymp}
\def\ati{{\underset{i}{\&}}}
\def\atieqz{{\underset{i=0}{\&}}}
\def\atilej{{\underset{i<j}{\&}}}
\def\atjneqi{{\underset{j\neq i}{\&}}}
\def\atmieqo{{\underset{i=1}{\overset{m}{\&}}}}
\def\atmieqz{{\underset{i=0}{\overset{m}{\&}}}}
\def\atzio{{\underset{i=1}{\overset{z}{\&}}}}
%\def\b{\beta}
\def\bobn{{b_1,\dots,b_n}}
\def\b1{\Box^{-1}}
\def\B1Bk{{B_1,\dots,B_k}}
\def\baB{\bar{\Box}}
\def\back{{\backslash}}
\def\baleph{{\tx{\hbox{\boldmath $\aleph$\unboldmath}}}}
\def\bafo{\bar{\forall}}
\def\baF{\overline{F}}
\def\baR{\overline{R}}
\def\bat{\overline{t}}
\def\bau{\overline{u}}
\def\bax{\overline{x}}
\def\bay{\overline{y}}
\def\baz{\overline{z}}
\def\bbe{\boldsymbol{1}}
\def\bbbe{{\boldsymbol{\beta}}}
%\def\bbigcapj{\boldsymbol{\bigcap_{\mathnormal{j\in J}}}}
%\def\bbigveej{\boldsymbol{\bigvee_{\mathnormal{j\in J}}}}
%\def\bbigwej{\boldsymbol{\bigwedge_{\mathnormal{j\in J}}}}
\def\bbigcapj{\boldsymbol{\bigcap_{\mbox{\scriptsize\unboldmath$ j\in J$}}}}
\def\bbigcupj{\boldsymbol{\bigcup_{\mbox{\scriptsize\unboldmath$ j\in J$}}}}
\def\bbigveea{\boldsymbol{\bigvee\limits_{\mbox{\scriptsize\unboldmath$ a\in D$}}}}
\def\bbigveec{\boldsymbol{\bigvee\limits_{\mbox{\scriptsize\unboldmath$ c\in D$}}}}
\def\bbigveed{\boldsymbol{\bigvee\limits_{\mbox{\scriptsize\unboldmath$ d\in D$}}}}
\def\bbigveej{\boldsymbol{\bigvee\limits_{\mbox{\scriptsize\unboldmath$ j\in J$}}}}
\def\bbigwec{\boldsymbol{\bigwedge\limits_{\mbox{\scriptsize\unboldmath$ c\in D$}}}}
\def\bbigwed{\boldsymbol{\bigwedge\limits_{\mbox{\scriptsize\unboldmath$ d\in D$}}}}
\def\bbigwej{\boldsymbol{\bigwedge\limits_{\mbox{\scriptsize\unboldmath$ j\in J$}}}}
\def\bbigwen{\boldsymbol{\bigwedge\limits_{\mbox{\scriptsize\unboldmath$ 1\leq i\leq n$}}}}
\def\bbn{\boldsymbol{0}}
\def\bbK4{{\bf K4}}
\def\bbD4{{\bf D4}}
\def\bbS4{{\bf S4}}
\def\bbw{\boldsymbol{\wedge}}
\def\bbx{\boldsymbol{\square}}
\def\bC{{\bf C}}
\def\bbc{{\tx{\bf {\em c}}}}
\def\bci{{{\tx{\bf {\em c}}_i}}}
\def\bCL{{\bf CL}}
\def\bcupmieqo{{\underset{i=1}{\overset{m}{\bigcup}}}}
\def\bD{{\bf D}}
\def\bD4{{\bf D4}}
\def\bdi{{\bf\Diamond}}
\def\be{\beta}
\def\bet{\beta}
\def\bfia{{\bfi{a}}}
\def\bfiaa{{\bfi{aa}}}
\def\bfiab{{\bfi{ab}}}
\def\bfib{{\bfi{b}}}
\def\bfic{{\bfi{c}}}
\def\bfix{{\bfi{x}}}
\def\bfa{{\bfi{a}}}
\def\bfb{{\bfi{b}}}
\def\bfc{{\bfi{c}}}
\def\bfd{{\bfi{d}}}
\def\bfPi{{\bfi{\Pi}}}
\def\bfv{{\bfi{v}}}
\def\bfmp{{\mbox{\boldmath $fmp$}}}
\def\bigv{\bigvee}
\def\bigw{\bigwedge}
\def\Bbi{{\mathbf i}}
\def\Bik{{B_{i,k}}}
\def\bIL{{\bf IL}}
\def\BJ{{\bf J}}
\def\bGr{{\bf Grz}}
\def\bGL{{\bf GL}}
\def\bK{{\bf K}}
\def\bbKt{{\bf K.t}}
\def\bL{{\tx{\bf {\em L}}}}
\def\bLa{{\bf \Lambda}}
\def\blacksquar{\rule{3mm}{3mm}}
\def\bmC{{\tx{\bf {\em C}}}}
\def\bmH{{\mbox{$\boldsymbol H$}}}
\def\bml{\boldmath\mbox{\bf L}\unboldmath}
\def\bML{{\bf ML}}
\def\bmP{{\tx{\bf {\em P}}}}
\def\bMT{{\bf MT}}
\def\bmu{{\boldsymbol{\mu}}}
\def\bmy{{\tx{\bf {\em y}}}}
\def\bo{{\mbox{\bf 1}}}
\def\BoBm{{B_0,\dots,B_m}}
\def\BoBn{{B_0,\dots,B_n}}
\def\bOm{\boldsymbol{\Omega}}
\def\bP{{\tx{\bf {\em P}}}}
\def\bPpn{{\tx{\bf {\em P}}^+_n}}
\def\bQCL{{\bf QCL}}
\def\bQH{{\bf QH}}
\def\bQK{{\bf QK}}
\def\bQS4{{\bf QS4}}
\def\brarrow{\mbox{$\mapsto$}}
\def\brho{\bar{\rho}}
\def\bSi{{\bf \Sigma}}
\def\Bsip{{B_{\sigma^+}}}
\def\bS5{{\bf S5}}
\def\BS5{{\bf S5}}
\def\bT{{\bf T}}
\def\bt{{\mbox{$\boldsymbol t$}}}
\def\bT{{\mbox{$\boldsymbol T$}}}
\def\bti{\blacksquare}
\def\Btia{{B_{t_{i_a}}}}
\def\btK{{\bf K.t}}
\def\Bto{{B_{t_1}}}
\def\bu{\bullet}
\def\bu{\bullet}
\def\bV{{\bf V}}
\def\BV{{\bf V}}
\def\bvee0{\bigvee}
\def\bvee{\boldsymbol{\vee}}
\def\bveej{{\underset{j}{\bigvee}}}
\def\bveejneqi{{\underset{j\neq i}{{\bigvee}}}}
\def\bveemieqo{{\underset{i=1}{\overset{m}{\bigvee}}}}
\def\bveenkeqo{{\underset{k=1}{\overset{n}{\bigvee}}}}
\def\bw{\bigwedge}
%\def\bx{\square}
\def\by{\boldsymbol{y}}
\def\Bz{{\bf z}}
\def\bz{{\tx{\bf {\em z}}}}
\def\C12{{\cal C}_1\t{\cal C}_2}
\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\CBK{{\cal BK}}
\def\cc{{\cal C}}
\def\cC{{\cal C}}
\def\CCK{{\cal CK}}
\def\cCn{{\cal C^{\fbox{\tiny$n$}}}}
\def\cCu{\cC^{\sqcup}}
\def\cd{\cdot}
\def\cD{{\cal D}}
\def\cDi{{{\cal D}_i}}
\def\cDj{{{\cal D}_j}}
\def\cDu{{\cal D}_u}
\def\cDv{{\cal D}_v}
\def\cE{{\cal E}}
\def\cF{{\cal F}}
\def\cFL{{{\cal F}_L}}
\def\cFQL{{{\cal F}_{QL}}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\chain{\overset{\Large\bullet}{\underset{\bullet}{\uph }}}
\def\ci{{c_{i}}}
\def\cik{{c_{i,k}}}
\def\Cik{{C_{i,k}}}
\def\cin{{c_{i_n}}}
\def\cio{{c_{i_1}}}
\def\circequiv{\stackrel{\circ}{\equiv}}
\def\cK{{\cal K}}
%\def\CK{{\kappa}}
\def\CK{{\mathcal Q}}
%\def\cl{\cal L}
\def\cL{{\cal L}}
\def\cLP{{\cal LP}}
\def\Clus{{\cal C}lus}
\def\cM{{\cal M}}
\def\cML{{{\cal M}_L}}
\def\cN{{\cal N}}
\def\cO{{\cal O}}
\def\cP{{\cal P}}
\def\CQ{{\cal Q}}
\def\cQB{{\cal QB}}
\def\cQK{{\cal QK}}
\def\cQP{{\cal QP}}
\def\cQW{{\cal QW}}
\def\cQZ{{\cal QZ}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\CU{{\cal U}}
\def\cV{{\cal V}}
\def\cur{\curlywedge}
\def\cW{{\cal W}}
\def\cX{{\cal X}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}
\def\d1{\Diamond^{-1}}
\def\da1aian{{a_1,\dots,a_i,\dots,a_n}}
\def\da1ban{{a_1,\dots,b,\dots,a_n}}
\def\da1n{{a_1,\dots,a_n}}
\def\dAlt{{\text{{\bf {\em Alt}}}}}
\def\dbar{\longrightarrow\!\! \rightarrow}
\def\dD{{\text{{\bf {\em D}}}}}
\def\DDL{{\BBD}}
\def\de{\delta}
\def\Del{{\Delta}}
\def\del{{\delta}}
\def\Deli{{\Delta_i}}
\def\den{\delta^{(1)}_n}
\def\deoiz{{\delta^{(1)}_{i_0}}}
\def\dFT{{\text{{\bf {\em FT}}}}}
\def\di{\Diamond}
\def\Di{\Diamond}
\def\DI{\ExtraBigDiamond}%{\largediamond}
\def\dK{{\text{{\bf {\em K}}}}}
\def\dkcs{\delta^{(k)}_*}
\def\dkee{\delta^{(k_1)}_1}
\def\dkke{\delta^{(k_2)}_1}
\def\dkn{\delta^{(k)}_n}
\def\dkne{\delta^{(k_n)}_1}
\def\dko{\delta^{(k)}_1}
\def\dL{{\text{{\bf {\em L}}}}}
\def\DLm{{D_{L,m}}}
\def\DLn{{D_{L,n}}}
\def\DLmo{{D_{L,m+1}}}
\def\DLno{{D_{L,n+1}}}
\def\DQLn{{D_{QL,n}}}
\def\dno{\delta^{(0)}_1}
\def\don{\delta^{(0)}_n}
\def\dri{\twoheadrightarrow}
\def\ds{\displaystyle}
\def\dS5{{\text{{\bf {\em S5}}}}}
\def\dSL{{\text{{\bf {\em SL}}}}}
\def\dv{\vdash}
\def\dx1n{\tx{\hbox{$x_1,\dots,x_n$}}}
\def\dx1yxn{{x_1,\dots,y,\dots,x_n}}
\def\Eg{{E.g.,\ }}
\def\eg{{e.g.\ }}
\def\egp{{e.g.}}
\def\emp{\varnothing}
\def\eqs{\eqslantless}
\def\eqv{\equiv}
\def\etal{{et al.\ }}
\def\etc{{etc.\ }}
\def\etcp{{etc}}
\def\ex{\exists}
\def\Fio{{F_i^0}}
\def\FmT{{Fm_T}}
\def\FmTak{{Fm_{T'_k}}}
\def\FmTal{{Fm_{T_\alpha}}}
\def\FmTfs{{Fm_{T^*}}}
\def\FmTi{{Fm_{T_i}}}
\def\FmTik{{Fm_{T_{i(k)}}}}
\def\FmTj{{Fm_{T_j}}}
\def\FmTs{{Fm_{T_*}}}
\def\FmTu{{Fm_{T_u}}}
\def\FmTz{{Fm_{T_0}}}
\def\fo{\forall}
\def\FozFkz{{F_1^0,\dots.F_k^0}}
\def\fr2{{\text{\scriptsize{\frame{2}}}}}
\def\fxf{F_1\ti\dots\times F_n}
\def\fxfn{\underbrace{F\ti\dots\times F}_{n\, {\rm times}}}
\def\gam{\gamma}
\def\Gam{\Gamma}
\def\Gamak{{\Gamma'_k}}
\def\Gami{\Gamma_i}
\def\Gamik{\Gamma_{i(k)}}
\def\Gamj{\Gamma_j}
\def\Gamo{{\Gamma_1}}
\def\Gi{\Gamma_i}
\def\Gj{\Gamma_j}
\def\Gu{\Gamma_u}
\def\Gv{\Gamma_v}
\def\Gz{\Gamma_0}
\def\I{\Phi}
\def\ie{{i.e.\ }}
\def\iep{{i.e.}}
\def\ieqom{{i=1,\dots,m}}
\def\Ii{\Phi_1}
\def\Ii{\Phi_1}
\def\Iii{\Phi_2}
\def\Isto{{(I^*_{t_1})}}
\def\Ite{{I_{t_1}}}
\def\Ito{{(I_{t_1})}}
\def\iztoib{{i_0,\dots,i_b}}
\def\jmo{{j_{m+1}}}
\def\jno{{j_{n+1}}}
%\def\L12{{\cal L}_1\t{\cal L}_2}
%\def\L12{{\cal L}_1\t{\cal L}_2}
\def\la{\lambda}
\def\La{\Lambda}
\def\lc{\lceil}
\def\LCC{{\bf L}({\cal C}_1\t{\cal C}_2)}
\def\LCLC{{\bf L}({\cal C}_1),{\bf L}({\cal C}_2)}
\def\ldot{\lessdot}
\def\leqLn{{\leq_{L,n}}}
\def\Li{\Leftarrow}
\def\lla{\langle}
\def\llbu{{}_\bullet^{\bullet}\mkern-12,5mu\mid\,}
\def\llbu{{}_\bullet^{\bullet}\mkern-12,5mu\mid\,}
\def\Ln{{L_n}}
\def\lo{\Diamond}
\def\Lo{{L^0}}
\def\lora{\longrightarrow}
\def\Lra{\Leftrightarrow}
\def\LRarr{{\Leftrightarrow}}
\def\lra{\Longrightarrow}
\def\lri{\Leftrightarrow}
\def\Lri{\Longleftrightarrow}
\def\LxL{\bL_1\ti\dots\times \bL_r}
\def\MF{\mathcal{F}}
\def\BBMf{{\rm \mathbb{M}}\tt{f}}
\def\miff{\;\mbox{iff}\;}
\def\mM{{\mathfrak{M}}}
\def\mbM{\mathbb{M}}
\def\mo{\vDash}
\def\mS{\mathbb{S}}
\def\mt{\mapsto}
\def\mud{{\mu_\delta}}
\def\nin{\not\in}
\def\nmo{{\,\not\mo\,}}
\def\nsb{{\!\bot}}
\def\o{\omega}
%\def\oB{\raisebox{.4ex}{\frac{\phantom{.}\!\phantom{.}}{\Box}}}
%\def\oB{\overline{\Box^{\phantom{X}}}}
\def\oB{\overline{\phantom{\mbox{\large J}}}\!\!\!\!\square}
\def\oD{\overline{\phantom{\mbox{\large J}}}\!\!\!\!\Diamond}
%\def\oD{\bar{\Diamond}}
\def\om{\omega}
\def\Om{\Omega}
\def\ot{\otimes}
\def\ora{\overrightarrow}
\def\p1pk{{p_1,\dots,p_k}}
\def\piLn{{\phi_{L,n}}}
\def\piQLn{{\phi_{QL,n}}}
\def\Pm{{P_m}}
\def\Pn{{P^n}}
\def\Pno{{P^{n+1}}}
\def\Po{{P^0}}
\def\pone{\pm}
\def\Ppn{{{\bf P}^+_n}}
\def\pu{{\rm pure}}
\def\qed{\rule{6pt}{6pt}}
%\def\r{\varrho}
\def\r1rn{{R_1,\dots,R_n}}
\def\r1rN{{R_1,\dots,R_N}}
\def\Ra{\Rightarrow}
\def\ReRn{{R_1,\dots,R_n}}
\def\ReRN{{R_1,\dots,R_N}}
\def\res{\!\upharpoonright\!}
%\def\Ri{\,\Rightarrow\,}
\def\ri{\rightarrow}
%\def\Ri{\Rightarrow}
\def\rr1n{{r_1,\dots,r_n}}
\def\rra{\rangle}
\def\rren{{r_1,\dots,r_n}}
\def\s1sn{{S_1,\dots,S_n}}
\def\sbq{\subseteq}
\def\sbw{\stackrel{\sim}{\subset}}
\def\scw {\stackrel{\centerdot}{\we}}
\def\sd{\mbox{sd}}
\def\sdf{\sd(F)}
\def\sdfx{\sd_F(x)}
\def\sdx{\sd(x)}
\def\SeSn{{S_1,\dots,S_n}}
\def\sht{{\prime}}
\def\sig{\sigma}
\def\Sig{\Sigma}
\def\sip{{\sigma^+}}
\def\sp{\supset}
\def\Sp{\Supset}
\def\spq{\supseteq}
\def\sqs{\sqsubset}
\def\sqbq{\sqsubseteq}
\def\sqr{\square}
\def\Sqr{\ExtraBigBox}%{\largesquare}
\def\ssb{\subset}
\def\sub{\mbox{sub}}
\def\t{\times}
\def\TabeGabe{{(T'_\beta,\Gamma'_\beta)}}
\def\TakGak{{(T'_k,\Gamma'_k)}}
\def\TalGal{{T_\alpha,\Gamma_\alpha}}
\def\tap{\thickapprox}
\def\tazto{{(t'_0,t_1)}}
\def\td{\nabla}
\def\td{\triangledown}
\def\tdo{\nabla}
\def\tF{\tilde{F}}
\def\TG{{(T,\Gamma)}}
\def\Th{\Theta}
\def\th{\theta}
\def\Thai{{\Theta'_i}}
\def\Thaiaa{{\Theta'_{i_{a'}}}}
\def\Thaiapo{{\Theta'_{i_{a+1}}}}
\def\Thaiz{{\Theta_{i_0}}}
\def\thc{{\ensuremath{\mbox{Th}{(\cC)}}}}
\def\thcn{\ensuremath{\mbox{Th}^n(\cC)}}
\def\Thi{{\Theta_i}}
\def\Thia{{\Theta_{i_a}}}
\def\Thiaa{{\Theta_{i_{a'}}}}
\def\Thiapo{{\Theta_{i_{a+1}}}}
\def\Thib{{\Theta'_{i_b}}}
\def\Thiz{{\Theta_{i_0}}}
\def\ti{\times}
\def\tia{{t_{i_a}}}
\def\tiaa{{t_{i_{a'}}}}
\def\TiGi{{(T_i,\Gamma_i)}}
\def\ToGo{{(T_1,\Gamma_1)}}
\def\ToMGoM{{(T_{0_M},\Gamma_{0_M})}}
\def\tR{\tilde{R}}
\def\ttR
{\tilde{\phantom{\mbox{\large J}}}\!\!\!\!\ R'}
\def\tu{\bigtriangleup}
\def\TuaGua{{(T_{u'},\Gamma_{u'})}}
\def\TualGual{{(T_{u_\alpha},\Gamma_{u_\alpha})}}
\def\TuGu{{(T_u,\Gamma_u)}}
\def\TujGuj{{(T_{u_j},\Gamma_{u_j})}}
\def\TvbeGvbe{{(T_{v_\beta},\Gamma_{v_\beta})}}
\def\TvGv{{(T_v,\Gamma_v)}}
\def\twha{\twoheadrightarrow}
\def\tW{\tilde{W}}
\def\tx{\text}
\def\TzGz{{(T_0,\Gamma_0)}}
\def\TzMGzM{{(T_{0_M},\Gamma_{0_M})}}
\def\tzto{{(t_0,t_1)}}
\def\tztt{{(t_0,t_1,t_2)}}
\def\Ua{{\bf a}}
\def\Ub{{\bf b}}
\def\ubr{\underbrace}
\def\Uc{{\bf c}}
\def\Ud{{\bf d}}
\def\undsub{\subseteqq}
\def\uP{{\underline{P}}}
\def\uR{{\underline{R}}}
\def\uph{\upharpoonright}
\def\Ups{\Upsilon}
\def\utr{\triangle}
\def\Ux{{\bf x}}
\def\Uy{{\bf y}}
\def\Uz{{\bf z}}
\def\va{\varepsilon}
\def\vas{\varsigma}
\def\vbsi{{\bfv_\sigma}}
\def\vd{\vdash}
\def\Vd{\Vdash}
\def\vh{\varrho}
\def\viz{{\em viz.,\ }}
\def\vmo{{v_{m+1}}}
\def\vno{{v_{n+1}}}
\def\vovm{{v_1,\dots,v_m}}
\def\vovn{{v_1,\dots,v_n}}
\def\vp{\varphi}
\def\vro{\varrho}
\def\vs{{\em vs.\ }}
\def\vsiovsim{{v_{\sigma(1)},\dots,v_{\sigma(m)}}}
\def\we{\wedge}
\def\wi{^{(=)}}
\def\Wtia{{W_{{t_i}_a}}}
\def\Wtib{{W_{{t_i}_b}}}
\def\xoxn{{x_1,\dots,x_n}}
\def\x1xn{{x_1,\dots,x_n}}
\def\xx1n{{x,x_1,\dots,x_n}}

\def\l1{\L}

%%ANNA (File1)
\def\bF{{\bfi{F}}}
\def\caL{{\cal L}}
\def\ds{{\displaystyle}}
\def\ra{\rightarrow}
\def\rarr{\rightarrow}
\def\Rarr{\Rightarrow}
\def\Larr{\Leftarrow}
\def\LLarr{{\Longleftarrow}}
\def\LRarr{{\Longrightarrow}}
\def\Ri0{{R_{i_0}}}
\def\Rie{{R_{i_1}}}
\def\Rik{{R_{i_k}}}
\def\Rika{{R_{i_m}}}
\def\Rj0{{R_{j_0}}}
\def\Rje{{R_{j_1}}}
\def\Rjm{{R_{j_m}}}
\def\Rn{{\bf R}^n}
\def\vap{{\varphi}}
\def\vapi0{{\varphi_{i_0}}}
\def\vapie{{\varphi_{i_1}}}
\def\vapik{{\varphi_{i_K}}}
\def\vapj0{{\varphi_{j_0}}}
\def\vapje{{\varphi_{j_1}}}
\def\vapjk{{\varphi_{j_K}}}

\newcommand\bfi[1]{\mathbf{#1}}
\newcommand\bmi[1]{\hbox{\textbf{\itshape #1}}}

%ANNA(dmitr1,2)
\def\aon{a_1,\dots,a_n}
%\def\rarr{\rightarrow}
%\def\Rarr{\Rightarrow}
\def\ruu{\rho_{uu}}
\def\ruv{\rho_{uv}}
\def\ruw{\rho_{uw}}
\def\rvw{\rho_{vw}}
\def\xon{x_1,\dots,x_n}
\def\ba{\mbox{$\boldsymbol{a}$}}
\def\bx{\mbox{$\boldsymbol{x}$}}
\def\bon{b_1,\dots,b_n}
\def\bon{b_1,\dots,b_n}
\def\don{d_1,\dots,d_n}
\def\von{v_1,\dots,v_n}
\def\yon{y_1,\dots,y_n}


%ANNA (Basic)


%\newcommand\bfi[1]{\hbox{\textbf{\itshape #1}}}
%\newcommand\bfi[1]{\mathbf{#1}}
%\newcommand{\bfi}[1]{\bf {#1}}
%\newtheorem{question}[theorem]{\rm QUESTION}

\def\azan{{a_0,\dots,a_n}}
%\def\bF{{\bfi{F}}}
\def\bfH{{\text{\bf H}}}
\def\bfJ{{\text{\bf J}}}
\def\bfL{{\text{\bf L}}}
\def\bfLD{{(\text{\bf L}+D)}}
\def\bfM{{\text{\bf M}}}
\def\bfN{{\text{\bf N}}}
\def\bfP{{\text{\bf P}}}
\def\bfPa{{\text{\bf P}$'$}}
\def\bfV{{\text{\bf V}}}
\def\caD{{\cal D}}
\def\cI{{\cal I}}
\def\cIs{{\cal I(\supset)}}
\def\cIsp{{\cal I(\supset,\perp)}}
\def\caL{{\cal L}}
\def\cL{{\cal L}}
\def\cF{{\cal F}}
\def\cocn{{c_1,\dots,c_n}}
\def\deoden{{\delta_1,\dots,\delta_n}}
\def\deovvden{{\delta_1\vee\dots\vee\delta_n}}
%\def\ds{{\displaystyle}}
\def\emp{{\varnothing}}
\def\Gaz{{\Gamma_0}}
\def\Gi{{\Gamma_i}}
\def\Gj{{\Gamma_j}}
\def\GaDe{{\Gamma,\Delta}}
\def\GazDez{{\Gamma_0,\Delta_0}}
\def\gaogam{{\gamma_1,\dots,\gamma_m}}
\def\GaoGan{{\Gamma_1,\dots,\Gamma_n}}
\def\gaowwgam{{\gamma_1\wedge\dots\wedge\gamma_m}}
%\def\ra{\rightarrow}
%\def\rarr{\rightarrow}
\def\lrarr{{\leftrightarrow}}
%\def\Rarr{\Rightarrow}
%\def\Larr{\Leftarrow}
%\def\LLarr{{\Longleftarrow}}
%\def\LRarr{{\Longrightarrow}}
\def\LLRarr{{\rightleftharpoons}}
\def\ova{{\overline{a}}}
\def\ovb{{\overline{b}}}
\def\ovF{{\overline{F}}}
\def\uarr{{\uparrow}}
\def\darr{{\downarrow}}
%\newcommand\vec[1]{\overrightarrow{#1}}

%Kripke-SL.tex

\newcommand{\Val}{\mbox{Val}}
\newcommand{\card}{\mbox{card}}
%\newcommand{\CF}{\mbox{$\mathcal{F}$}}
%\newcommand{\CL}{\mbox{$\mathcal{L}$}}
%\newcommand{\CM}{\mbox{$\mathcal{M}$}}


%% added by Jane 4.2.03
\newcommand{\ILeaF}{\mbox{${\bf IL}'^{(=)}(\BBF)$}}
\newcommand{\ILeF}{\mbox{${\bf IL}^{(=)}(\BBF)$}}
\newcommand{\ILF}{\mbox{${\bf IL}(\BBF)$}}
\newcommand{\laxr}{\mbox{$\jsem{\Ba/\Bx}$}}
\newcommand{\ovRsn}{\mbox{$\overline{R}^*_n$}}
\newcommand{\MLeF}{\mbox{${\bf ML}^{(=)}(\BBF)$}}
\newcommand{\RsN}{\mbox{$R\_ n$}}
\newcommand{\lbxr}{\mbox{$\jsem{\Bb/\Bx}$}}
\newcommand{\laaxr}{\mbox{$\jsem{\Ba'/\Bx}$}}
\newcommand{\QH}{{\bf QH}}
\newcommand{\IL}{{\bf IL}}
%\newcommand{\BS}{{\bf S}}
\newcommand{\ML}{{\bf ML}}
\newcommand{\Rsn}{\Bc R^*_n\Bc}
\newcommand{\lcaxr}{\jsem{\Bc'/\Bx}}


\def\vare{{\varepsilon}}
\def\sym{{\sim}}
%\newcommand{\BBa}{\mbox{\(\Bbb a\)}}
\def\bPi{{\bf\Pi}}
\def\BBa{{\bf a}}
\def\BBx{{\bf x}}
\def\BBy{{\bf y}}
\def\bI{{\bf I}}

%ANNA spring 2005 (Ch. 6)
\def\inv{{\text{\rm \small inv}}}
\newcommand{\bsML}{{\boldsymbol{M}\hspace{-1mm}\boldsymbol{L}}}
\def\FI{{(\BBF,\overline{I})}}
\newcommand{\bsa}{{\boldsymbol{a}}}
\newcommand{\bsx}{{\boldsymbol{x}}}
\def\bpi{{\bar{\pi}}}
\newcommand{\bsb}{{\boldsymbol{b}}}
\newcommand{\bsB}{{\boldsymbol{B}}}
\newcommand{\bsc}{{\boldsymbol{c}}}
\newcommand{\bsC}{{\boldsymbol{C}}}
\newcommand{\bsd}{{\boldsymbol{d}}}
\newcommand{\bsh}{{\boldsymbol{h}}}
\newcommand{\bsH}{{\boldsymbol{H}}}
\newcommand{\bsL}{{\boldsymbol{L}}}
\def\tI{\text{$\tilde{I}\,$}}
\newcommand{\Zm}{Z_M}
\newcommand{\ZmF}[1]{\Zm(#1, \bot)}

\def\r1rN{{R_1,\dots,R_N}}

\newlength{\JaneDepth}
\newlength{\JaneWidth}

\newcommand{\jane}[1]{%
  \settodepth{\JaneDepth}{\ensuremath{#1}}%
  \addtolength{\JaneDepth}{.4ex}%
  \settowidth{\JaneWidth}{\ensuremath{#1}}%
  \addtolength{\JaneWidth}{.75ex}%
  \ensuremath{%
    \mathop{%
      \makebox[0pt][l]{%
      \rule[-\the\JaneDepth]{.4pt}{.5ex}%
      \rule[-\the\JaneDepth]{\the\JaneWidth}{.4pt}%
      \rule[-\the\JaneDepth]{.4pt}{.5ex}}%
      \makebox[\JaneWidth][l]{%
        \hspace{.5ex}\ensuremath{#1}}%
      }%
  }%
}



%---------[ILSH:begin]--------

% "Figure N:" to "Figure N."

\makeatletter
\long\def\@makecaption#1#2{%
   \vskip 10\p@
   \setbox\@tempboxa\hbox{#1. #2}%
   \ifdim \wd\@tempboxa >\hsize
       #1. #2\par
     \else
       \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
   \fi}
\makeatother


%---------[ILSH:end]--------


